Biased Tales: Cultural and Topic Bias in Generating Children's Stories

Stories play a pivotal role in human communication, shaping beliefs and morals, particularly in children. As parents increasingly rely on large language models (LLMs) to craft bedtime stories, the presence of cultural and gender stereotypes in these narratives raises significant concerns. To address this issue, we present Biased Tales, a comprehensive dataset designed to analyze how biases influence protagonists' attributes and story elements in LLM-generated stories. Our analysis uncovers striking disparities. When the protagonist is described as a girl (as compared to a boy), appearance-related attributes increase by 55.26%. Stories featuring non-Western children disproportionately emphasize cultural heritage, tradition, and family themes far more than those for Western children. Our findings highlight the role of sociocultural bias in making creative AI use more equitable and diverse.

==> generated/corr_protagonist_attributes_gender_of_child.tex <==
\null\\[-1.7em]
\multicolumn{2}{l}{\bf Gender Of Child} \\
child & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} little } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} fur } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} soft } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} shimmering } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} coat } { {\fontsize{7}{7}\selectfont 5\%} hopeful } \\
daughter & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} hair } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 8\%} black } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 8\%} gentle } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} immaginative } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} bright } { {\fontsize{7}{7}\selectfont 5\%} loving } \\
son & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 14\%} young } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} adventurous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} hero } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} brave } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} eager } { {\fontsize{7}{7}\selectfont 5\%} wise } \\
\bottomrule\\


==> generated/corr_protagonist_attributes_model.tex <==
\null\\[-1.7em]
\multicolumn{2}{l}{\bf Model} \\

GPT4 & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 14\%} dreamer } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 14\%} hearted } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 12\%} courageous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} special } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} big } { {\fontsize{7}{7}\selectfont 10\%} determined } \\
Llama3 & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 14\%} hair } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 14\%} wanderer } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} black } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} welcomed } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} awaited } { {\fontsize{7}{7}\selectfont 8\%} gentle } \\
\bottomrule\\


==> generated/corr_protagonist_attributes_nationality_parent_developed.tex <==
\null\\[-1.7em]
\multicolumn{2}{l}{\bf Nationality Parent Developed} \\

Developed & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} suprised } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} friendly } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} little } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} fur } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} helpful } { {\fontsize{7}{7}\selectfont 4\%} golden } \\
Developing & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} young } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 8\%} wise } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} sparkling } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} loved } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} black } { {\fontsize{7}{7}\selectfont 4\%} leader } \\
\bottomrule\\


==> generated/corr_protagonist_attributes_nationality_parent_group.tex <==
\null\\[-1.7em]
\multicolumn{2}{l}{\bf Nationality Parent Group} \\

Africa & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 10\%} wise } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} clever } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} spirit } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} decisive } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} young } { {\fontsize{7}{7}\selectfont 4\%} respectful } \\
Asia & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 10\%} pure } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} gentle } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} chosen } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} kind } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} loving } { {\fontsize{7}{7}\selectfont 5\%} hearted } \\
European & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} friendly } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} suprised } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} golden } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} drawn } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} warm } { {\fontsize{7}{7}\selectfont 4\%} imaginative } \\
Middle Eastern & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 8\%} young } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} hero } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} wide } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} proud } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} courageous } { {\fontsize{7}{7}\selectfont 3\%} challenged } \\
North American & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} suprised } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} thrilled } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} tiny } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} excited } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} dreamer } { {\fontsize{7}{7}\selectfont 3\%} imaginative } \\
South American & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 8\%} joyous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} wings } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} sparkling } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} tiny } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} eyes } { {\fontsize{7}{7}\selectfont 5\%} guardian } \\
\bottomrule\\


==> generated/corr_protagonist_attributes_race_of_parent.tex <==
\null\\[-1.7em]
\multicolumn{2}{l}{\bf Race Of Parent} \\

African-Amer. & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 38\%} heritage } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 34\%} proud } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 28\%} connected } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 26\%} strong } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 23\%} inspired } { {\fontsize{7}{7}\selectfont 23\%} purposeful } \\
Asian & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 15\%} wise } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 15\%} noble } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} kind } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} peaceful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} perseverant } { {\fontsize{7}{7}\selectfont 11\%} hearted } \\
European-Amer. & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 19\%} golden } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 17\%} blue } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 15\%} friendly } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} open } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} brave } { {\fontsize{7}{7}\selectfont 13\%} observant } \\
Latino & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 27\%} oriented } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 25\%} family } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 16\%} sparkling } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 16\%} loving } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} connected } { {\fontsize{7}{7}\selectfont 12\%} eyes } \\
Middle-Eastern & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 20\%} wise } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 14\%} generous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} selfless } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} compassionate } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 12\%} weaver } { {\fontsize{7}{7}\selectfont 10\%} clever } \\
White & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 21\%} friendly } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 16\%} helpful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 15\%} empathetic } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} blue } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 10\%} brown } { {\fontsize{7}{7}\selectfont 10\%} grateful } \\
\bottomrule\\


==> generated/corr_protagonist_attributes_religion_of_parent.tex <==
\null\\[-1.7em]
\multicolumn{2}{l}{\bf Religion Of Parent} \\

Atheist & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 46\%} minded } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 45\%} inquisitive } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 36\%} open } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 31\%} nature } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 28\%} observant } { {\fontsize{7}{7}\selectfont 25\%} connected } \\
Buddhist & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 40\%} mindful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 33\%} understanding } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 31\%} peaceful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 31\%} compassionate } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 21\%} empathetic } { {\fontsize{7}{7}\selectfont 18\%} patient } \\
Christian & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 39\%} faithful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 32\%} trusting } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 32\%} loving } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 27\%} caring } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 15\%} hopeful } { {\fontsize{7}{7}\selectfont 14\%} peaceful } \\
Hindu & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 22\%} pure } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 17\%} respectful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 16\%} magical } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 16\%} selfless } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 15\%} wise } { {\fontsize{7}{7}\selectfont 12\%} brave } \\
Jew & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 48\%} heritage } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 42\%} tradition } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 30\%} family } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 27\%} oriented } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 23\%} excitable } { {\fontsize{7}{7}\selectfont 22\%} proud } \\
Muslim & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 26\%} faithful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 21\%} grateful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 19\%} devoted } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 18\%} patient } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 17\%} kind } { {\fontsize{7}{7}\selectfont 16\%} spiritual } \\
\bottomrule\\


==> generated/corr_protagonist_attributes_role_of_parent.tex <==
\null\\[-1.7em]
\multicolumn{2}{l}{\bf Role Of Parent} \\

father & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} decisive } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} wise } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} explorer } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} protector } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} amazed } { {\fontsize{7}{7}\selectfont 4\%} celebrated } \\
mother & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} dear } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} coat } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} free } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} loved } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} soft } { {\fontsize{7}{7}\selectfont 4\%} tiny } \\
parent & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} careful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} spirited } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} magical } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} connected } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 3\%} understanding } { {\fontsize{7}{7}\selectfont 3\%} grateful } \\
\bottomrule\\


==> generated/corr_story_text_lemmas_model.tex <==
\null\\[-1.7em]
\multicolumn{2}{l}{\bf Model} \\

GPT4 & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 44\%} end } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 42\%} vast } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 39\%} time } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 35\%} home } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 24\%} way } { {\fontsize{7}{7}\selectfont 24\%} shared } \\
Llama3 & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 56\%} bedtime } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 45\%} scent } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 27\%} hidden } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 26\%} secret } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 26\%} air } { {\fontsize{7}{7}\selectfont 26\%} sleep } \\
\bottomrule\\


==> generated/frequency_categories_stories.tex <==

\begin{table*}[ht]
\centering
\small
\begin{tabular}{llccccc}
\toprule
source\_column & source\_value & trait\_physical & trait\_emotional & trait\_mental & trait\_moral & trait\_other \\
\midrule
country & Afghanistan & 121 & 258 & 334 & 198 & 39 \\
country & Armenia & 129 & 241 & 297 & 209 & 52 \\
country & Azerbaijan & 120 & 253 & 321 & 166 & 52 \\
country & Brazil & 149 & 281 & 360 & 125 & 61 \\
country & China & 74 & 278 & 297 & 212 & 43 \\
country & Egypt & 109 & 213 & 382 & 154 & 58 \\
country & Ethiopia & 123 & 246 & 339 & 174 & 27 \\
country & Germany & 151 & 281 & 303 & 152 & 54 \\
country & Great Britain & 788 & 1722 & 1551 & 1030 & 278 \\
country & India & 90 & 238 & 357 & 188 & 35 \\
country & Indonesia & 106 & 258 & 306 & 183 & 26 \\
country & Iran & 121 & 265 & 321 & 176 & 43 \\
country & Iraq & 106 & 229 & 356 & 164 & 31 \\
country & Italy & 574 & 1556 & 1880 & 986 & 241 \\
country & Japan & 90 & 267 & 277 & 182 & 29 \\
country & Kenya & 130 & 259 & 349 & 164 & 52 \\
country & Mali & 106 & 206 & 339 & 190 & 41 \\
country & Mexico & 117 & 274 & 301 & 158 & 39 \\
country & Nigeria & 74 & 201 & 354 & 205 & 23 \\
country & Philippines & 89 & 251 & 309 & 185 & 41 \\
country & Russia & 152 & 289 & 274 & 151 & 46 \\
country & South Africa & 145 & 268 & 378 & 144 & 40 \\
country & Sri Lanka & 95 & 282 & 325 & 152 & 37 \\
country & Sudan & 99 & 244 & 304 & 176 & 35 \\
country & Tajikistan & 105 & 243 & 316 & 183 & 44 \\
country & Thailand & 128 & 302 & 253 & 177 & 45 \\
country & United States & 679 & 1579 & 1678 & 962 & 338 \\
country & Vietnam & 132 & 290 & 312 & 163 & 43 \\ 
\midrule
ethnicity & African-American & 207 & 285 & 443 & 183 & 81 \\
ethnicity & Asian & 92 & 283 & 303 & 220 & 32 \\
ethnicity & European-American & 143 & 252 & 350 & 165 & 69 \\
ethnicity & Latino & 164 & 291 & 334 & 154 & 75 \\
ethnicity & Middle-Eastern & 124 & 239 & 336 & 201 & 32 \\
ethnicity & White & 166 & 300 & 270 & 177 & 55 \\
\midrule
gender & child & 1694 & 3756 & 4290 & 2291 & 726 \\
gender & daughter & 1937 & 4073 & 3814 & 2513 & 648 \\
gender & son & 1271 & 3445 & 5069 & 2505 & 519 \\
\midrule
religion & Atheist & 104 & 319 & 436 & 108 & 68 \\
religion & Buddhist & 60 & 444 & 316 & 177 & 24 \\
religion & Christian & 1580 & 3580 & 4156 & 2283 & 592 \\
religion & Hindu & 1452 & 3132 & 4198 & 2342 & 510 \\
religion & Jew & 72 & 271 & 259 & 203 & 65 \\
religion & Muslim & 1634 & 3528 & 3808 & 2196 & 634 \\
\midrule
role & father & 1452 & 3132 & 4198 & 2342 & 510 \\
role & mother & 1634 & 3528 & 3808 & 2196 & 634 \\
role & parent & 1580 & 3580 & 4156 & 2283 & 592 \\
\bottomrule
\end{tabular}
\caption{The frequency of character-centric attributes for each sociocultural factors.}
\label{tab:character-ferquency}
\end{table*}


==> generated/frequency_variables_stories.tex <==

\begin{table*}[ht]
\centering
\small
% \resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccccc}
\toprule
% Sociocultural &  Sociocultural &  Geolocation &  Geolocation & Geolocation &Geolocation &  Geolocation &  Urbun &  Urbun &  Urbun &  Social & Social &  Social\\
% factor & value & Desert & Green Bodies & Magical/Imaginary & Mountain & Water Bodies & City & Town & Village & Middle-class & Poor & Wealthy \\
\multirow{2}{*}{\textbf{Factor}} & \multirow{2}{*}{\textbf{value}} & \multicolumn{5}{c}{\textbf{Geo-location}} & \multicolumn{3}{c}{\textbf{Urban}} & \multicolumn{3}{c}{\textbf{Social}} \\
\cmidrule(lr){3-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
 &  & \emoji{desert} & \emoji{evergreen-tree} & \emoji{magic-wand} & \emoji{snow-capped-mountain} & \emoji{water-wave} & \emoji{cityscape} & \emoji{circus-tent} & \emoji{house-with-garden} & \emoji{money-bag}& \emoji{money-bag}\emoji{money-bag} & \emoji{money-bag}\emoji{money-bag}\emoji{money-bag}  \\
 % &  & Desert\emoji{desert} & Green B.\emoji{evergreen-tree} & Magical\emoji{magic-wand} & Mountain\emoji{snow-capped-mountain} & Water B.\emoji{water-wave} & City\emoji{cityscape} & Town\emoji{circus-tent} & Village\emoji{house-with-garden} & Middle-class & Poor & Wealthy \\

\midrule
% \midrule
      country &       Afghanistan &                   3 &                        16 &                                     8 &                   102 &                         0 &          21 &           0 &             93 &            4 &                   35 &               6 \\
      country &           Armenia &                   0 &                        22 &                                     5 &                   106 &                         2 &           6 &           2 &             99 &            2 &                   23 &               5 \\
      country &        Azerbaijan &                   1 &                        37 &                                     4 &                    76 &                        15 &          17 &           1 &             87 &            1 &                   30 &               7 \\
      country &            Brazil &                   0 &                       124 &                                     8 &                     0 &                         2 &           6 &          14 &             34 &            1 &                    3 &               0 \\
      country &             China &                   0 &                        38 &                                    14 &                    80 &                         1 &           1 &           0 &            119 &            9 &                   19 &               0 \\
      country &             Egypt &                  82 &                         0 &                                     3 &                     0 &                        40 &          43 &           1 &             50 &            2 &                   29 &              21 \\
      country &          Ethiopia &                   2 &                        62 &                                     9 &                    59 &                         2 &           6 &           0 &             94 &            8 &                   10 &               4 \\
      country &           Germany &                   0 &                       111 &                                    12 &                    10 &                         2 &           1 &           4 &            105 &            0 &                   26 &               1 \\
      country &     Great Britain &                  40 &                       291 &                                   261 &                   100 &                        10 &          20 &          23 &            411 &           11 &                  108 &              86 \\
      country &             India &                   2 &                        74 &                                    13 &                    30 &                         5 &           3 &           1 &            113 &            5 &                   17 &               7 \\
      country &         Indonesia &                   0 &                       120 &                                     9 &                     4 &                         1 &           1 &           1 &             93 &            3 &                   19 &               1 \\
      country &              Iran &                  21 &                        29 &                                    38 &                    35 &                         2 &          35 &           4 &             50 &            2 &                   28 &              22 \\
      country &              Iraq &                  56 &                        18 &                                    20 &                     0 &                        34 &          62 &           1 &             47 &            2 &                   32 &               9 \\
      country &             Italy &                  44 &                       336 &                                   173 &                   132 &                         9 &          31 &          41 &            460 &           13 &                  141 &              40 \\
      country &             Japan &                   0 &                        64 &                                    15 &                    54 &                         1 &           0 &           4 &            111 &            2 &                   15 &               0 \\
      country &             Kenya &                   1 &                       102 &                                     0 &                    30 &                         1 &           0 &           0 &             78 &            4 &                    4 &               0 \\
      country &              Mali &                  44 &                        68 &                                     2 &                     2 &                        14 &           5 &           0 &            108 &           11 &                    6 &               0 \\
      country &            Mexico &                   7 &                        75 &                                    14 &                    29 &                         4 &           1 &          16 &             94 &            6 &                   21 &               0 \\
      country &           Nigeria &                   0 &                       118 &                                     7 &                     0 &                         3 &           4 &           2 &            111 &            7 &                    9 &               0 \\
      country &       Philippines &                   0 &                        93 &                                     8 &                    20 &                        11 &           2 &           8 &            104 &           17 &                    7 &               0 \\
      country &            Russia &                   0 &                        75 &                                    38 &                    12 &                         1 &           1 &           0 &             95 &            3 &                   19 &               2 \\
      country &      South Africa &                   2 &                        80 &                                    11 &                    35 &                         3 &           1 &           0 &             58 &            5 &                    7 &               1 \\
      country &         Sri Lanka &                   0 &                       106 &                                     4 &                    15 &                        10 &           1 &           0 &             88 &            1 &                   12 &               4 \\
      country &             Sudan &                  71 &                        28 &                                     8 &                     4 &                        20 &           7 &           0 &             69 &            9 &                    3 &               1 \\
      country &        Tajikistan &                   0 &                         0 &                                     1 &                   134 &                         0 &           0 &           3 &            106 &            4 &                   15 &               2 \\
      country &          Thailand &                   0 &                       115 &                                     8 &                     8 &                         2 &           7 &           0 &             66 &            3 &                   14 &               7 \\
      country &     United States &                  47 &                       239 &                                   286 &                   107 &                        12 &          26 &          49 &            338 &           17 &                   90 &              36 \\
      country &           Vietnam &                   0 &                        99 &                                     4 &                    16 &                        11 &           7 &           0 &            113 &            8 &                   28 &               0 \\ \midrule
    ethnicity &  African-American &                   2 &                        90 &                                    35 &                     1 &                         2 &          11 &           5 &             72 &            2 &                    7 &              10 \\
    ethnicity &             Asian &                   0 &                        68 &                                    28 &                    38 &                         1 &           0 &           0 &            108 &            5 &                   26 &               3 \\
    ethnicity & European-American &                   0 &                        67 &                                    55 &                    10 &                         3 &           2 &           5 &             88 &            0 &                   26 &              14 \\
    ethnicity &            Latino &                   1 &                        59 &                                    18 &                    50 &                         3 &           0 &          11 &            118 &            5 &                   26 &               0 \\
    ethnicity &    Middle-Eastern &                 103 &                         2 &                                    12 &                     4 &                         5 &          37 &           5 &             66 &            6 &                   28 &              26 \\
    ethnicity &             White &                   0 &                        30 &                                   100 &                     3 &                         1 &           0 &           4 &             26 &            0 &                   17 &              26 \\ \midrule
       gender &             child &                 141 &                       844 &                                   330 &                   402 &                        70 &          91 &          63 &           1073 &           53 &                  226 &              57 \\
       gender &          daughter &                 148 &                       846 &                                   376 &                   358 &                        66 &         104 &          47 &           1146 &           49 &                  255 &             143 \\
       gender &               son &                 134 &                       850 &                                   277 &                   440 &                        82 &         120 &          65 &           1175 &           58 &                  289 &              62 \\ \midrule
     religion &           Atheist &                   0 &                        25 &                                    84 &                    11 &                         0 &           4 &           3 &             31 &            0 &                    7 &               3 \\
     religion &          Buddhist &                   0 &                        39 &                                    17 &                    74 &                         5 &           2 &           0 &            102 &            3 &                    5 &               2 \\
     religion &         Christian &                 126 &                       817 &                                   320 &                   338 &                        67 &         108 &          60 &           1044 &           51 &                  250 &              73 \\
     religion &             Hindu &                 141 &                       781 &                                   274 &                   384 &                        75 &         100 &          54 &           1052 &           47 &                  266 &             112 \\
     religion &               Jew &                   1 &                        79 &                                     5 &                    32 &                         0 &           3 &           6 &            123 &            7 &                   34 &               1 \\
     religion &            Muslim &                 155 &                       799 &                                   283 &                   361 &                        71 &          98 &          52 &           1042 &           52 &                  208 &              71 \\ \midrule
         role &            father &                 141 &                       781 &                                   274 &                   384 &                        75 &         100 &          54 &           1052 &           47 &                  266 &             112 \\
         role &            mother &                 155 &                       799 &                                   283 &                   361 &                        71 &          98 &          52 &           1042 &           52 &                  208 &              71 \\
         role &            parent &                 126 &                       817 &                                   320 &                   338 &                        67 &         108 &          60 &           1044 &           51 &                  250 &              73 \\
\bottomrule
\end{tabular}

% }
\caption{The frequency of context-centric attributes for each sociocultural factors\\ (Desert: \emoji{desert}, Green Bodies: \emoji{evergreen-tree}, Magical: \emoji{magic-wand}, Mountain: \emoji{snow-capped-mountain}, Water Bodies: \emoji{water-wave}, City: \emoji{cityscape}, Town:\emoji{circus-tent}, Village:\emoji{house-with-garden}, Middle-class:\emoji{money-bag}\emoji{money-bag} , Poor: \emoji{money-bag}, Wealthy:\emoji{money-bag}\emoji{money-bag}\emoji{money-bag}).}
\label{tab:context-ferquency}
\end{table*}
% VZ: This is amazing!

==> generated/frequency_variables_stories_colors.tex <==
\begin{table*}[ht]
\centering
\small
\begin{tabular}{llccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Factor}} & \multirow{2}{*}{\textbf{value}} & \multicolumn{5}{c}{\textbf{Geo-location}} & \multicolumn{3}{c}{\textbf{Urban}} & \multicolumn{3}{c}{\textbf{Social}} \\
\cmidrule(lr){3-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
 &  & \emoji{desert} & \emoji{evergreen-tree} & \emoji{magic-wand} & \emoji{snow-capped-mountain} & \emoji{water-wave} & \emoji{cityscape} & \emoji{circus-tent} & \emoji{house-with-garden} & \emoji{money-bag}& \emoji{money-bag}\emoji{money-bag} & \emoji{money-bag}\emoji{money-bag}\emoji{money-bag}  \\
\midrule
      country &       Afghanistan & \cellcolor{red!20}3 & 16 & 8 & \cellcolor{green!20}102 & \cellcolor{red!20}0 & \cellcolor{green!20}21 & \cellcolor{red!20}0 & 93 & 4 & \cellcolor{green!20}35 & 6 \\
      country &           Armenia & \cellcolor{red!20}0 & 22 & 5 & \cellcolor{green!20}106 & 2 & 6 & 2 & \cellcolor{green!20}99 & 2 & 23 & 5 \\
      country &        Azerbaijan & 1 & 37 & 4 & \cellcolor{green!20}76 & 15 & \cellcolor{green!20}17 & 1 & 87 & 1 & \cellcolor{green!20}30 & 7 \\
      country &            Brazil & \cellcolor{red!20}0 & \cellcolor{green!20}124 & 8 & \cellcolor{red!20}0 & 2 & 6 & \cellcolor{green!20}14 & 34 & 1 & 3 & \cellcolor{red!20}0 \\
      country &             China & \cellcolor{red!20}0 & 38 & 14 & 80 & 1 & \cellcolor{red!20}1 & \cellcolor{red!20}0 & \cellcolor{green!20}119 & 9 & 19 & \cellcolor{red!20}0 \\
      country &             Egypt & \cellcolor{green!20}82 & \cellcolor{red!20}0 & 3 & \cellcolor{red!20}0 & 40 & \cellcolor{green!20}43 & 1 & 50 & 2 & 29 & \cellcolor{green!20}21 \\
      country &          Ethiopia & 2 & \cellcolor{green!20}62 & 9 & 59 & 2 & 6 & \cellcolor{red!20}0 & \cellcolor{green!20}94 & 8 & 10 & 4 \\
      country &           Germany & \cellcolor{red!20}0 & \cellcolor{green!20}111 & 12 & 10 & 2 & 1 & 4 & \cellcolor{green!20}105 & \cellcolor{red!20}0 & 26 & 1 \\
      country &     Great Britain & 40 & 291 & \cellcolor{green!20}261 & 100 & 10 & 20 & 23 & \cellcolor{green!20}411 & 11 & \cellcolor{green!20}108 & 86 \\
      country &             India & 2 & 74 & 13 & 30 & 5 & \cellcolor{red!20}3 & 1 & \cellcolor{green!20}113 & 5 & 17 & 7 \\
      country &         Indonesia & \cellcolor{red!20}0 & \cellcolor{green!20}120 & 9 & 4 & 1 & 1 & 1 & \cellcolor{green!20}93 & 3 & 19 & 1 \\
      country &              Iran & 21 & 29 & 38 & 35 & 2 & \cellcolor{green!20}35 & 4 & 50 & 2 & 28 & \cellcolor{green!20}22 \\
      country &              Iraq & \cellcolor{green!20}56 & 18 & 20 & \cellcolor{red!20}0 & 34 & \cellcolor{green!20}62 & 1 & 47 & 2 & 32 & 9 \\
      country &             Italy & 44 & \cellcolor{green!20}336 & \cellcolor{green!20}173 & 132 & 9 & 31 & 41 & \cellcolor{green!20}460 & 13 & \cellcolor{green!20}141 & 40 \\
      country &             Japan & \cellcolor{red!20}0 & 64 & 15 & 54 & 1 & \cellcolor{red!20}0 & 4 & \cellcolor{green!20}111 & 2 & 15 & \cellcolor{red!20}0 \\
      country &             Kenya & 1 & \cellcolor{green!20}102 & \cellcolor{red!20}0 & 30 & 1 & \cellcolor{red!20}0 & \cellcolor{red!20}0 & 78 & 4 & 4 & \cellcolor{red!20}0 \\
      country &              Mali & \cellcolor{green!20}44 & 68 & 2 & 2 & 14 & 5 & \cellcolor{red!20}0 & \cellcolor{green!20}108 & 11 & 6 & \cellcolor{red!20}0 \\
      country &            Mexico & 7 & 75 & 14 & 29 & 4 & \cellcolor{red!20}1 & \cellcolor{green!20}16 & 94 & 6 & 21 & \cellcolor{red!20}0 \\
      country &           Nigeria & \cellcolor{red!20}0 & \cellcolor{green!20}118 & 7 & \cellcolor{red!20}0 & 3 & 4 & 2 & \cellcolor{green!20}111 & 7 & 9 & \cellcolor{red!20}0 \\
      country &       Philippines & \cellcolor{red!20}0 & 93 & 8 & 20 & 11 & 2 & 8 & \cellcolor{green!20}104 & \cellcolor{green!20}17 & 7 & \cellcolor{red!20}0 \\
      country &            Russia & \cellcolor{red!20}0 & 75 & 38 & 12 & 1 & 1 & \cellcolor{red!20}0 & 95 & 3 & 19 & 2 \\
      country &      South Africa & 2 & 80 & 11 & 35 & 3 & 1 & \cellcolor{red!20}0 & 58 & 5 & 7 & 1 \\
      country &         Sri Lanka & \cellcolor{red!20}0 & \cellcolor{green!20}106 & 4 & 15 & 10 & 1 & \cellcolor{red!20}0 & 88 & 1 & 12 & 4 \\
      country &             Sudan & \cellcolor{green!20}71 & 28 & 8 & 4 & 20 & 7 & \cellcolor{red!20}0 & 69 & 9 & 3 & 1 \\
      country &        Tajikistan & \cellcolor{red!20}0 & \cellcolor{red!20}0 & 1 & \cellcolor{green!20}134 & \cellcolor{red!20}0 & \cellcolor{red!20}0 & 3 & \cellcolor{green!20}106 & 4 & 15 & 2 \\
      country &          Thailand & \cellcolor{red!20}0 & \cellcolor{green!20}115 & 8 & 8 & 2 & 7 & \cellcolor{red!20}0 & 66 & 3 & 14 & 7 \\
      country &     United States & 47 & 239 & \cellcolor{green!20}286 & 107 & 12 & 26 & \cellcolor{green!20}49 & \cellcolor{green!20}338 & 17 & 90 & 36 \\
      country &           Vietnam & \cellcolor{red!20}0 & \cellcolor{green!20}99 & 4 & 16 & 11 & 7 & \cellcolor{red!20}0 & \cellcolor{green!20}113 & 8 & 28 & \cellcolor{red!20}0 \\
    ethnicity &  African-American & 2 & 90 & 35 & 1 & 2 & \cellcolor{green!20}11 & 5 & 72 & 2 & 7 & \cellcolor{green!20}10 \\
    ethnicity &             Asian & \cellcolor{red!20}0 & 68 & 28 & 38 & 1 & \cellcolor{red!20}0 & \cellcolor{red!20}0 & \cellcolor{green!20}108 & 5 & 26 & 3 \\
    ethnicity & European-American & \cellcolor{red!20}0 & 67 & 55 & 10 & 3 & 2 & 5 & 88 & \cellcolor{red!20}0 & 26 & \cellcolor{green!20}14 \\
    ethnicity &            Latino & 1 & 59 & 18 & 50 & 3 & \cellcolor{red!20}0 & \cellcolor{green!20}11 & \cellcolor{green!20}118 & 5 & 26 & \cellcolor{red!20}0 \\
    ethnicity &    Middle-Eastern & \cellcolor{green!20}103 & 2 & 12 & 4 & 5 & \cellcolor{green!20}37 & 5 & 66 & 6 & 28 & \cellcolor{green!20}26 \\
    ethnicity &             White & \cellcolor{red!20}0 & 30 & \cellcolor{green!20}100 & 3 & 1 & \cellcolor{red!20}0 & 4 & 26 & \cellcolor{red!20}0 & 17 & \cellcolor{green!20}26 \\
       gender &             child & \cellcolor{green!20}141 & 844 & 330 & 402 & 70 & 91 & 63 & \cellcolor{green!20}1073 & 53 & 226 & 57 \\
       gender &          daughter & \cellcolor{green!20}148 & 846 & 376 & 358 & 66 & 104 & 47 & \cellcolor{green!20}1146 & 49 & 255 & \cellcolor{green!20}143 \\
       gender &               son & \cellcolor{red!20}134 & 850 & 277 & \cellcolor{green!20}440 & 82 & \cellcolor{green!20}120 & 65 & \cellcolor{green!20}1175 & 58 & \cellcolor{green!20}289 & 62 \\
     religion &           Atheist & \cellcolor{red!20}0 & 25 & \cellcolor{green!20}84 & 11 & \cellcolor{red!20}0 & 4 & 3 & 31 & \cellcolor{red!20}0 & 7 & 3 \\
     religion &          Buddhist & \cellcolor{red!20}0 & 39 & 17 & \cellcolor{green!20}74 & 5 & 2 & \cellcolor{red!20}0 & \cellcolor{green!20}102 & 3 & 5 & 2 \\
     religion &         Christian & 126 & 817 & 320 & 338 & 67 & 108 & 60 & \cellcolor{green!20}1044 & 51 & 250 & 73 \\
     religion &             Hindu & \cellcolor{green!20}141 & 781 & 274 & \cellcolor{green!20}384 & 75 & 100 & 54 & \cellcolor{green!20}1052 & 47 & 266 & \cellcolor{green!20}112 \\
     religion &               Jew & 1 & 79 & 5 & 32 & \cellcolor{red!20}0 & 3 & 6 & \cellcolor{green!20}123 & 7 & 34 & 1 \\
     religion &            Muslim & \cellcolor{green!20}155 & 799 & 283 & 361 & 71 & 98 & 52 & \cellcolor{green!20}1042 & 52 & 208 & 71 \\
         role &            father & \cellcolor{green!20}141 & 781 & 274 & \cellcolor{green!20}384 & 75 & 100 & 54 & \cellcolor{green!20}1052 & 47 & 266 & \cellcolor{green!20}112 \\
         role &            mother & \cellcolor{green!20}155 & 799 & 283 & 361 & 71 & 98 & 52 & \cellcolor{green!20}1042 & 52 & 208 & 71 \\
         role &            parent & 126 & 817 & 320 & 338 & 67 & 108 & 60 & \cellcolor{green!20}1044 & 51 & 250 & 73 \\
\bottomrule
\end{tabular}
\caption{The frequency of context-centric attributes for each sociocultural factors\\ (Desert: \emoji{desert}, Green Bodies: \emoji{evergreen-tree}, Magical: \emoji{magic-wand}, Mountain: \emoji{snow-capped-mountain}, Water Bodies: \emoji{water-wave}, City: \emoji{cityscape}, Town:\emoji{circus-tent}, Village:\emoji{house-with-garden}, Middle-class:\emoji{money-bag}\emoji{money-bag} , Poor: \emoji{money-bag}, Wealthy:\emoji{money-bag}\emoji{money-bag}\emoji{money-bag}).}
\label{tab:context-ferquency}
\end{table*}

==> generated/percentage_variable_stories.tex <==

\begin{table*}[ht]
\centering
\tiny
% \resizebox{\textwidth}{!}{%
\begin{tabular}{ll|cccccc|cccc|ccccc}
\toprule

\multirow{2}{*}{\textbf{Factor}} & \multirow{2}{*}{\textbf{value}} & \multicolumn{6}{c}{\textbf{Geo-location}} & \multicolumn{4}{c}{\textbf{Urban}} & \multicolumn{4}{c}{\textbf{Social}} \\
 &   &  \emoji{desert} &  \emoji{evergreen-tree} & \emoji{magic-wand} &  \emoji{snow-capped-mountain} &  \emoji{water-wave} & \emoji{cross-mark} &  \emoji{house-with-garden}  &  \emoji{circus-tent} &  \emoji{cityscape} &  \emoji{cross-mark} &  \emoji{money-bag} & \emoji{money-bag}\emoji{money-bag} &  \emoji{money-bag}\emoji{money-bag}\emoji{money-bag} &  \emoji{cross-mark} \\
\midrule
      country &       Afghanistan &                 2.2 &                      11.9 &                                   5.9 &                  75.6 &                       0.0 &               4.4 &           68.9 &         0.0 &        15.6 &        15.6 &          3.0 &                 25.9 &             4.4 &         66.7 \\
      country &           Armenia &                 0.0 &                      16.3 &                                   3.7 &                  78.5 &                       1.5 &               0.0 &           73.3 &         1.5 &         4.4 &        20.7 &          1.5 &                 17.0 &             3.7 &         77.8 \\
      country &        Azerbaijan &                 0.7 &                      27.4 &                                   3.0 &                  56.3 &                      11.1 &               1.5 &           64.4 &         0.7 &        12.6 &        22.2 &          0.7 &                 22.2 &             5.2 &         71.9 \\
      country &            Brazil &                 0.0 &                      91.9 &                                   5.9 &                   0.0 &                       1.5 &               0.7 &           25.2 &        10.4 &         4.4 &        60.0 &          0.7 &                  2.2 &             0.0 &         97.0 \\
      country &             China &                 0.0 &                      28.1 &                                  10.4 &                  59.3 &                       0.7 &               1.5 &           88.1 &         0.0 &         0.7 &        11.1 &          6.7 &                 14.1 &             0.0 &         79.3 \\
      country &             Egypt &                60.7 &                       0.0 &                                   2.2 &                   0.0 &                      29.6 &               7.4 &           37.0 &         0.7 &        31.9 &        30.4 &          1.5 &                 21.5 &            15.6 &         61.5 \\
      country &          Ethiopia &                 1.5 &                      45.9 &                                   6.7 &                  43.7 &                       1.5 &               0.7 &           69.6 &         0.0 &         4.4 &        25.9 &          5.9 &                  7.4 &             3.0 &         83.7 \\
      country &           Germany &                 0.0 &                      82.2 &                                   8.9 &                   7.4 &                       1.5 &               0.0 &           77.8 &         3.0 &         0.7 &        18.5 &          0.0 &                 19.3 &             0.7 &         80.0 \\
      country &     Great Britain &                 5.6 &                      40.4 &                                  36.2 &                  13.9 &                       1.4 &               2.5 &           57.1 &         3.2 &         2.8 &        36.9 &          1.5 &                 15.0 &            11.9 &         71.5 \\
      country &             India &                 1.5 &                      54.8 &                                   9.6 &                  22.2 &                       3.7 &               8.1 &           83.7 &         0.7 &         2.2 &        13.3 &          3.7 &                 12.6 &             5.2 &         78.5 \\
      country &         Indonesia &                 0.0 &                      88.9 &                                   6.7 &                   3.0 &                       0.7 &               0.7 &           68.9 &         0.7 &         0.7 &        29.6 &          2.2 &                 14.1 &             0.7 &         83.0 \\
      country &              Iran &                15.6 &                      21.5 &                                  28.1 &                  25.9 &                       1.5 &               7.4 &           37.0 &         3.0 &        25.9 &        34.1 &          1.5 &                 20.7 &            16.3 &         61.5 \\
      country &              Iraq &                41.5 &                      13.3 &                                  14.8 &                   0.0 &                      25.2 &               5.2 &           34.8 &         0.7 &        45.9 &        18.5 &          1.5 &                 23.7 &             6.7 &         68.1 \\
      country &             Italy &                 6.1 &                      46.7 &                                  24.0 &                  18.3 &                       1.2 &               3.6 &           63.9 &         5.7 &         4.3 &        26.1 &          1.8 &                 19.6 &             5.6 &         73.1 \\
      country &             Japan &                 0.0 &                      47.4 &                                  11.1 &                  40.0 &                       0.7 &               0.7 &           82.2 &         3.0 &         0.0 &        14.8 &          1.5 &                 11.1 &             0.0 &         87.4 \\
      country &             Kenya &                 0.7 &                      75.6 &                                   0.0 &                  22.2 &                       0.7 &               0.7 &           57.8 &         0.0 &         0.0 &        42.2 &          3.0 &                  3.0 &             0.0 &         94.1 \\
      country &              Mali &                32.6 &                      50.4 &                                   1.5 &                   1.5 &                      10.4 &               3.7 &           80.0 &         0.0 &         3.7 &        16.3 &          8.1 &                  4.4 &             0.0 &         87.4 \\
      country &            Mexico &                 5.2 &                      55.6 &                                  10.4 &                  21.5 &                       3.0 &               4.4 &           69.6 &        11.9 &         0.7 &        17.8 &          4.4 &                 15.6 &             0.0 &         80.0 \\
      country &           Nigeria &                 0.0 &                      87.4 &                                   5.2 &                   0.0 &                       2.2 &               5.2 &           82.2 &         1.5 &         3.0 &        13.3 &          5.2 &                  6.7 &             0.0 &         88.1 \\
      country &       Philippines &                 0.0 &                      68.9 &                                   5.9 &                  14.8 &                       8.1 &               2.2 &           77.0 &         5.9 &         1.5 &        15.6 &         12.6 &                  5.2 &             0.0 &         82.2 \\
      country &            Russia &                 0.0 &                      55.6 &                                  28.1 &                   8.9 &                       0.7 &               6.7 &           70.4 &         0.0 &         0.7 &        28.9 &          2.2 &                 14.1 &             1.5 &         82.2 \\
      country &      South Africa &                 1.5 &                      59.3 &                                   8.1 &                  25.9 &                       2.2 &               3.0 &           43.0 &         0.0 &         0.7 &        56.3 &          3.7 &                  5.2 &             0.7 &         90.4 \\
      country &         Sri Lanka &                 0.0 &                      78.5 &                                   3.0 &                  11.1 &                       7.4 &               0.0 &           65.2 &         0.0 &         0.7 &        34.1 &          0.7 &                  8.9 &             3.0 &         87.4 \\
      country &             Sudan &                52.6 &                      20.7 &                                   5.9 &                   3.0 &                      14.8 &               3.0 &           51.1 &         0.0 &         5.2 &        43.7 &          6.7 &                  2.2 &             0.7 &         90.4 \\
      country &        Tajikistan &                 0.0 &                       0.0 &                                   0.7 &                  99.3 &                       0.0 &               0.0 &           78.5 &         2.2 &         0.0 &        19.3 &          3.0 &                 11.1 &             1.5 &         84.4 \\
      country &          Thailand &                 0.0 &                      85.2 &                                   5.9 &                   5.9 &                       1.5 &               1.5 &           48.9 &         0.0 &         5.2 &        45.9 &          2.2 &                 10.4 &             5.2 &         82.2 \\
      country &     United States &                 6.5 &                      33.2 &                                  39.7 &                  14.9 &                       1.7 &               4.0 &           46.9 &         6.8 &         3.6 &        42.6 &          2.4 &                 12.5 &             5.0 &         80.1 \\
      country &           Vietnam &                 0.0 &                      73.3 &                                   3.0 &                  11.9 &                       8.1 &               3.7 &           83.7 &         0.0 &         5.2 &        11.1 &          5.9 &                 20.7 &             0.0 &         73.3 \\
      \midrule
    ethnicity &  African-Amer. &                 1.5 &                      66.7 &                                  25.9 &                   0.7 &                       1.5 &               3.7 &           53.3 &         3.7 &         8.1 &        34.8 &          1.5 &                  5.2 &             7.4 &         85.9 \\
    ethnicity &             Asian &                 0.0 &                      50.4 &                                  20.7 &                  28.1 &                       0.7 &               0.0 &           80.0 &         0.0 &         0.0 &        20.0 &          3.7 &                 19.3 &             2.2 &         74.8 \\
    ethnicity & European-Amer. &                 0.0 &                      49.6 &                                  40.7 &                   7.4 &                       2.2 &               0.0 &           65.2 &         3.7 &         1.5 &        29.6 &          0.0 &                 19.3 &            10.4 &         70.4 \\
    ethnicity &            Latino &                 0.7 &                      43.7 &                                  13.3 &                  37.0 &                       2.2 &               3.0 &           87.4 &         8.1 &         0.0 &         4.4 &          3.7 &                 19.3 &             0.0 &         77.0 \\
    ethnicity &    Middle-East. &                76.3 &                       1.5 &                                   8.9 &                   3.0 &                       3.7 &               6.7 &           48.9 &         3.7 &        27.4 &        20.0 &          4.4 &                 20.7 &            19.3 &         55.6 \\
    ethnicity &             White &                 0.0 &                      22.2 &                                  74.1 &                   2.2 &                       0.7 &               0.7 &           19.3 &         3.0 &         0.0 &        77.8 &          0.0 &                 12.6 &            19.3 &         68.1 \\
    \midrule
       gender &             child &                 7.6 &                      45.7 &                                  17.9 &                  21.8 &                       3.8 &               3.1 &           58.2 &         3.4 &         4.9 &        33.5 &          2.9 &                 12.2 &             3.1 &         81.8 \\
       gender &          daughter &                 8.0 &                      45.9 &                                  20.4 &                  19.4 &                       3.6 &               2.8 &           62.1 &         2.5 &         5.6 &        29.7 &          2.7 &                 13.8 &             7.8 &         75.8 \\
       gender &               son &                 7.3 &                      46.1 &                                  15.0 &                  23.8 &                       4.4 &               3.4 &           63.7 &         3.5 &         6.5 &        26.3 &          3.1 &                 15.7 &             3.4 &         77.8 \\
       \midrule
     religion &           Atheist &                 0.0 &                      18.5 &                                  62.2 &                   8.1 &                       0.0 &              11.1 &           23.0 &         2.2 &         3.0 &        71.9 &          0.0 &                  5.2 &             2.2 &         92.6 \\
     religion &          Buddhist &                 0.0 &                      28.9 &                                  12.6 &                  54.8 &                       3.7 &               0.0 &           75.6 &         0.0 &         1.5 &        23.0 &          2.2 &                  3.7 &             1.5 &         92.6 \\
     religion &         Christian &                 7.4 &                      47.8 &                                  18.7 &                  19.8 &                       3.9 &               2.5 &           61.1 &         3.5 &         6.3 &        29.1 &          3.0 &                 14.6 &             4.3 &         78.1 \\
     religion &             Hindu &                 8.2 &                      45.7 &                                  16.0 &                  22.5 &                       4.4 &               3.2 &           61.5 &         3.2 &         5.8 &        29.5 &          2.7 &                 15.6 &             6.5 &         75.1 \\
     religion &               Jew &                 0.7 &                      58.5 &                                   3.7 &                  23.7 &                       0.0 &              13.3 &           91.1 &         4.4 &         2.2 &         2.2 &          5.2 &                 25.2 &             0.7 &         68.9 \\
     religion &            Muslim &                 9.1 &                      46.7 &                                  16.5 &                  21.1 &                       4.2 &               2.4 &           60.9 &         3.0 &         5.7 &        30.3 &          3.0 &                 12.2 &             4.2 &         80.6 \\
     \midrule
         role &            father &                 8.2 &                      45.7 &                                  16.0 &                  22.5 &                       4.4 &               3.2 &           61.5 &         3.2 &         5.8 &        29.5 &          2.7 &                 15.6 &             6.5 &         75.1 \\
         role &            mother &                 9.1 &                      46.7 &                                  16.5 &                  21.1 &                       4.2 &               2.4 &           60.9 &         3.0 &         5.7 &        30.3 &          3.0 &                 12.2 &             4.2 &         80.6 \\
         role &            parent &                 7.4 &                      47.8 &                                  18.7 &                  19.8 &                       3.9 &               2.5 &           61.1 &         3.5 &         6.3 &        29.1 &          3.0 &                 14.6 &             4.3 &         78.1 \\
\bottomrule

\end{tabular}

% }
\caption{The percentage of context-centric attributes for each sociocultural factors\\ (Desert: \emoji{desert}, Green Bodies: \emoji{evergreen-tree}, Magical: \emoji{magic-wand}, Mountain: \emoji{snow-capped-mountain}, Water Bodies: \emoji{water-wave}, City: \emoji{cityscape}, Town:\emoji{circus-tent}, Village:\emoji{house-with-garden}, Middle-class:\emoji{money-bag}\emoji{money-bag} , Poor: \emoji{money-bag}, Wealthy:\emoji{money-bag}\emoji{money-bag}\emoji{money-bag}, Not found=\emoji{cross-mark}.)}
\label{tab:context-percentage}
\end{table*}
% VZ: This is amazing!

==> generated/std_categories.tex <==
\begin{table*}
\begin{tabular}{llccccc}
\toprule
Factor & Value & trait\_physical & trait\_emotional & trait\_mental & trait\_moral & trait\_other \\
\midrule
country & Afghanistan & 0.160 & 0.186 & 0.198 & 0.190 & 0.070 \\
country & Armenia & 0.157 & 0.179 & 0.204 & 0.185 & 0.100 \\
country & Azerbaijan & 0.162 & 0.176 & 0.201 & 0.167 & 0.099 \\
country & Brazil & 0.169 & 0.182 & 0.182 & 0.146 & 0.101 \\
country & China & 0.120 & 0.197 & 0.197 & 0.175 & 0.103 \\
country & Egypt & 0.136 & 0.182 & 0.228 & 0.153 & 0.119 \\
country & Ethiopia & 0.155 & 0.208 & 0.185 & 0.149 & 0.065 \\
country & Germany & 0.173 & 0.206 & 0.201 & 0.152 & 0.097 \\
country & Great Britain & 0.163 & 0.192 & 0.196 & 0.166 & 0.091 \\
country & India & 0.130 & 0.179 & 0.188 & 0.159 & 0.072 \\
country & Indonesia & 0.154 & 0.192 & 0.188 & 0.182 & 0.071 \\
country & Iran & 0.153 & 0.184 & 0.203 & 0.154 & 0.081 \\
country & Iraq & 0.151 & 0.193 & 0.212 & 0.198 & 0.067 \\
country & Italy & 0.143 & 0.197 & 0.204 & 0.175 & 0.092 \\
country & Japan & 0.153 & 0.213 & 0.177 & 0.163 & 0.074 \\
country & Kenya & 0.148 & 0.188 & 0.201 & 0.177 & 0.088 \\
country & Mali & 0.151 & 0.180 & 0.181 & 0.200 & 0.095 \\
country & Mexico & 0.167 & 0.196 & 0.206 & 0.156 & 0.082 \\
country & Nigeria & 0.122 & 0.194 & 0.200 & 0.195 & 0.054 \\
country & Philippines & 0.143 & 0.184 & 0.175 & 0.172 & 0.099 \\
country & Russia & 0.166 & 0.213 & 0.202 & 0.140 & 0.091 \\
country & South Africa & 0.154 & 0.193 & 0.197 & 0.148 & 0.077 \\
country & Sri Lanka & 0.153 & 0.208 & 0.199 & 0.171 & 0.089 \\
country & Sudan & 0.151 & 0.195 & 0.197 & 0.195 & 0.087 \\
country & Tajikistan & 0.146 & 0.198 & 0.198 & 0.185 & 0.101 \\
country & Thailand & 0.158 & 0.198 & 0.182 & 0.150 & 0.093 \\
country & United States & 0.157 & 0.199 & 0.196 & 0.180 & 0.104 \\
country & Vietnam & 0.165 & 0.191 & 0.203 & 0.170 & 0.079 \\
\midrule
ethnicity & African-American & 0.153 & 0.166 & 0.188 & 0.134 & 0.083 \\
ethnicity & Asian & 0.131 & 0.186 & 0.191 & 0.189 & 0.082 \\
ethnicity & European-American & 0.165 & 0.210 & 0.216 & 0.168 & 0.123 \\
ethnicity & Latino & 0.179 & 0.198 & 0.189 & 0.160 & 0.109 \\
ethnicity & Middle-Eastern & 0.149 & 0.169 & 0.191 & 0.180 & 0.073 \\
ethnicity & White & 0.163 & 0.194 & 0.190 & 0.153 & 0.108 \\
\midrule
gender & child & 0.156 & 0.194 & 0.196 & 0.179 & 0.099 \\
gender & daughter & 0.172 & 0.198 & 0.194 & 0.163 & 0.089 \\
gender & son & 0.127 & 0.191 & 0.196 & 0.176 & 0.084 \\
\midrule
religion & Atheist & 0.123 & 0.181 & 0.193 & 0.125 & 0.094 \\
religion & Buddhist & 0.099 & 0.176 & 0.170 & 0.128 & 0.069 \\
religion & Christian & 0.156 & 0.195 & 0.202 & 0.177 & 0.088 \\
religion & Hindu & 0.152 & 0.192 & 0.203 & 0.173 & 0.088 \\
religion & Jew & 0.114 & 0.185 & 0.192 & 0.178 & 0.131 \\
religion & Muslim & 0.161 & 0.196 & 0.196 & 0.172 & 0.094 \\
\midrule
role & father & 0.152 & 0.192 & 0.203 & 0.173 & 0.088 \\
role & mother & 0.161 & 0.196 & 0.196 & 0.172 & 0.094 \\
role & parent & 0.156 & 0.195 & 0.202 & 0.177 & 0.088 \\
\bottomrule
\end{tabular}
\caption{Standard Deviations of Normalized Trait Proportions by Identity Factor}
\label{tab:trait_std}
\end{table*}

==> generated_GPT4/corr_protagonist_gpt4_model.tex <==
\null\\[-1.7em]
\multicolumn{2}{l}{\bf Model} \\

GPT4 & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} adventure } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} adventurous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} awe } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} beautiful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} big } { {\fontsize{7}{7}\selectfont nan\%} blue } \\
\bottomrule\\


==> generated_GPT4/corr_story_text_lemmas_model.tex <==
\null\\[-1.7em]
\multicolumn{2}{l}{\bf Model} \\

GPT4 & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} ali } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} amina } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} amir } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} awaited } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} away } { {\fontsize{7}{7}\selectfont nan\%} began } \\
\bottomrule\\


==> generated_Llama3/corr_protagonist_gpt4_model.tex <==
\null\\[-1.7em]
\multicolumn{2}{l}{\bf Model} \\

llama3 & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} adventure } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} adventurous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} amazed } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} awe } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} beautiful } { {\fontsize{7}{7}\selectfont nan\%} big } \\
\bottomrule\\


==> generated_Llama3/corr_story_text_lemmas_model.tex <==
\null\\[-1.7em]
\multicolumn{2}{l}{\bf Model} \\

llama3 & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} ah } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} appeared } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} approached } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} asked } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} bedtime } { {\fontsize{7}{7}\selectfont nan\%} began } \\
\bottomrule\\


==> generated_Mixtral8x/corr_protagonist_gpt4_model.tex <==
\null\\[-1.7em]
\multicolumn{2}{l}{\bf Model} \\

Mixtral8x & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} adventurous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} amazed } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} animal } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} appreciative } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} awe } { {\fontsize{7}{7}\selectfont nan\%} beautiful } \\
\bottomrule\\


==> generated_Mixtral8x/corr_story_text_lemmas_model.tex <==
\null\\[-1.7em]
\multicolumn{2}{l}{\bf Model} \\

Mixtral8x & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} ada } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} adventurous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} aisha } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} ali } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont nan\%} approached } { {\fontsize{7}{7}\selectfont nan\%} away } \\
\bottomrule\\


==> generated_unmasked/corr_protagonist_gpt4_ethnicity.tex <==
\null\\[-2.5em]
\multicolumn{2}{l}{\bf Ethnicity} \\

African-Amer. & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 37\%} strong } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 29\%} skin } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 27\%} resilient } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 21\%} courageous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 20\%} dark } { {\fontsize{7}{7}\selectfont 18\%} powerful } \\
Asian & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 22\%} gentle } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 16\%} peaceful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 12\%} skilled } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 12\%} compassionate } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 10\%} overjoyed } { {\fontsize{7}{7}\selectfont 10\%} helpful } \\
European-Amer. & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 16\%} blue } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} american } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} special } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 10\%} brown } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 10\%} eye } { {\fontsize{7}{7}\selectfont 10\%} animal } \\
Latino & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 17\%} black } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 17\%} magic } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 14\%} curly } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 14\%} big } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} felt } { {\fontsize{7}{7}\selectfont 13\%} brown } \\
Middle-Eastern & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 19\%} generous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 14\%} eyed } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} wise } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} eyes } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 10\%} clever } { {\fontsize{7}{7}\selectfont 9\%} imaginative } \\
White & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 28\%} white } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 21\%} blue } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 17\%} golden } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 16\%} sparkling } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} eye } { {\fontsize{7}{7}\selectfont 9\%} beautiful } \\
\bottomrule\\


==> generated_unmasked/corr_protagonist_gpt4_gender.tex <==
\null\\[-2.5em]
\multicolumn{2}{l}{\bf Gender} \\

child & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} playful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} little } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} grateful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} friend } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} helpful } { {\fontsize{7}{7}\selectfont 3\%} loved } \\
daughter & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 18\%} hair } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 17\%} beautiful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 14\%} gentle } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 12\%} kind } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} bright } { {\fontsize{7}{7}\selectfont 11\%} smile } \\
son & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 15\%} brave } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 12\%} curious } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} young } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 10\%} adventurous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 8\%} courageous } { {\fontsize{7}{7}\selectfont 6\%} eager } \\
\bottomrule\\


==> generated_unmasked/corr_protagonist_gpt4_model.tex <==
\null\\[-2.5em]
\multicolumn{2}{l}{\bf Model} \\

GPT4 & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 17\%} young } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 15\%} safe } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 14\%} grateful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} kindness } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 12\%} big } { {\fontsize{7}{7}\selectfont 12\%} courageous } \\
Mixtral8x & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 39\%} kind } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 22\%} learn } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 22\%} determined } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 21\%} overjoyed } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 20\%} wise } { {\fontsize{7}{7}\selectfont 19\%} caring } \\
llama3 & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 30\%} hair } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 28\%} bright } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 24\%} black } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 23\%} wonder } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 22\%} eyes } { {\fontsize{7}{7}\selectfont 22\%} star } \\
\bottomrule\\


==> generated_unmasked/corr_protagonist_gpt4_nationality_parent_developed.tex <==
\null\\[-2.5em]
\multicolumn{2}{l}{\bf Nationality Parent Developed} \\

Developed & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 12\%} blue } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} gentle } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} golden } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} loving } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} compassionate } { {\fontsize{7}{7}\selectfont 7\%} peaceful } \\
Developing & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} black } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} adventurous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} brave } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} determined } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} curious } { {\fontsize{7}{7}\selectfont 5\%} pure } \\
\bottomrule\\


==> generated_unmasked/corr_protagonist_gpt4_nationality_parent_group.tex <==
\null\\[-2.5em]
\multicolumn{2}{l}{\bf Nationality Parent Group} \\

Africa & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} adventurous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} curiosity } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} brave } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} bright } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} connected } { {\fontsize{7}{7}\selectfont 3\%} black } \\
Asia & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} kind } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} respectful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} hearted } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} playful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} content } { {\fontsize{7}{7}\selectfont 4\%} black } \\
European & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 14\%} blue } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} golden } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} hair } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} gentle } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} beautiful } { {\fontsize{7}{7}\selectfont 6\%} eye } \\
Middle Eastern & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} eyed } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} young } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} brave } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} courageous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} imaginative } { {\fontsize{7}{7}\selectfont 4\%} story } \\
North American & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} explore } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} loving } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} nature } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} helpful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} compassionate } { {\fontsize{7}{7}\selectfont 3\%} friend } \\
South American & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} little } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} curious } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} playful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} adventurous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} black } { {\fontsize{7}{7}\selectfont 3\%} gift } \\
\bottomrule\\


==> generated_unmasked/corr_protagonist_gpt4_religion.tex <==
\null\\[-2.5em]
\multicolumn{2}{l}{\bf Religion} \\

Atheist & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 10\%} awe } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} sense } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} connection } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} peace } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} wonder } { {\fontsize{7}{7}\selectfont 6\%} imaginative } \\
Buddhist & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 23\%} compassionate } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 22\%} understanding } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 19\%} peaceful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} wise } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} gentle } { {\fontsize{7}{7}\selectfont 9\%} loving } \\
Christian & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} eye } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} joyful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} deep } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 3\%} love } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 3\%} amazed } { {\fontsize{7}{7}\selectfont 3\%} curious } \\
Hindu & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} brave } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} strong } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} courageous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} adventurous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 3\%} clever } { {\fontsize{7}{7}\selectfont 3\%} wise } \\
Jew & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} wise } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} proud } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} loving } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} generous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} kind } { {\fontsize{7}{7}\selectfont 3\%} wisdom } \\
Muslim & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} little } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} loved } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 3\%} special } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 3\%} filled } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 3\%} happy } { {\fontsize{7}{7}\selectfont 3\%} golden } \\
\bottomrule\\


==> generated_unmasked/corr_protagonist_gpt4_role.tex <==
\null\\[-2.5em]
\multicolumn{2}{l}{\bf Role} \\

 & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 16\%} understanding } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 15\%} compassionate } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} peaceful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} wise } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} peace } { {\fontsize{7}{7}\selectfont 7\%} loving } \\
father & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} brave } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} strong } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} courageous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} adventurous } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 3\%} clever } { {\fontsize{7}{7}\selectfont 3\%} wise } \\
mother & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} little } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} loved } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 3\%} special } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 3\%} filled } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 3\%} happy } { {\fontsize{7}{7}\selectfont 3\%} golden } \\
parent & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} eye } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} joyful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} deep } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 3\%} love } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 3\%} amazed } { {\fontsize{7}{7}\selectfont 3\%} curious } \\
\bottomrule\\


==> generated_unmasked/corr_story_text_lemmas_ethnicity.tex <==
\null\\[-2.5em]
\multicolumn{2}{l}{\bf Ethnicity} \\

African-Amer. & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 66\%} kofi } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 34\%} ada } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 20\%} powerful } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 19\%} remember } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} taught } { {\fontsize{7}{7}\selectfont 9\%} shared } \\
Asian & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 57\%} mei } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 26\%} lin } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 24\%} ling } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 15\%} nestled } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} overjoyed } { {\fontsize{7}{7}\selectfont 9\%} continued } \\
European-Amer. & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 21\%} owl } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 20\%} fox } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 19\%} clearing } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 19\%} oliver } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 19\%} sophie } { {\fontsize{7}{7}\selectfont 18\%} lily } \\
Latino & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 38\%} mateo } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 35\%} diego } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 29\%} nestled } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 25\%} maria } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 23\%} isabella } { {\fontsize{7}{7}\selectfont 18\%} sofia } \\
Middle-Eastern & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 68\%} middle } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 66\%} dune } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 36\%} layla } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 26\%} karim } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 25\%} hassan } { {\fontsize{7}{7}\selectfont 25\%} leila } \\
White & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 37\%} lily } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 14\%} edge } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} leo } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 12\%} owl } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} matter } { {\fontsize{7}{7}\selectfont 10\%} set } \\
\bottomrule\\


==> generated_unmasked/corr_story_text_lemmas_gender.tex <==
\null\\[-2.5em]
\multicolumn{2}{l}{\bf Gender} \\

child & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} owl } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} high } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} decided } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} fox } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 3\%} thanked } { {\fontsize{7}{7}\selectfont 3\%} shared } \\
daughter & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 20\%} lily } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 12\%} layla } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} dear } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 10\%} amina } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} sofia } { {\fontsize{7}{7}\selectfont 8\%} aisha } \\
son & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 10\%} ali } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 8\%} encountered } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 8\%} set } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} mysterious } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} max } { {\fontsize{7}{7}\selectfont 7\%} leo } \\
\bottomrule\\


==> generated_unmasked/corr_story_text_lemmas_model.tex <==
\null\\[-2.5em]
\multicolumn{2}{l}{\bf Model} \\

GPT4 & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 52\%} drifted } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 25\%} end } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 25\%} evening } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 23\%} tucked } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 21\%} knowing } { {\fontsize{7}{7}\selectfont 19\%} sat } \\
Mixtral8x & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 34\%} overjoyed } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 32\%} spent } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 26\%} looked } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 23\%} finally } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 22\%} soon } { {\fontsize{7}{7}\selectfont 21\%} near } \\
llama3 & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 49\%} wore } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 33\%} suddenly } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 32\%} wandered } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 31\%} guide } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 28\%} returned } { {\fontsize{7}{7}\selectfont 27\%} led } \\
\bottomrule\\


==> generated_unmasked/corr_story_text_lemmas_nationality_parent_developed.tex <==
\null\\[-2.5em]
\multicolumn{2}{l}{\bf Nationality Parent Developed} \\

Developed & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 23\%} lily } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 18\%} nestled } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 14\%} fox } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} owl } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 10\%} max } { {\fontsize{7}{7}\selectfont 10\%} leo } \\
Developing & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 19\%} monkey } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} near } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 8\%} ali } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 8\%} waterfall } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 8\%} fruit } { {\fontsize{7}{7}\selectfont 6\%} granted } \\
\bottomrule\\


==> generated_unmasked/corr_story_text_lemmas_nationality_parent_group.tex <==
\null\\[-2.5em]
\multicolumn{2}{l}{\bf Nationality Parent Group} \\

Africa & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 12\%} kofi } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} horizon } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} ada } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} amina } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 8\%} monkey } { {\fontsize{7}{7}\selectfont 7\%} gathered } \\
Asia & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 16\%} monkey } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 12\%} waterfall } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 12\%} rohan } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} near } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 10\%} mei } { {\fontsize{7}{7}\selectfont 6\%} decided } \\
European & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 16\%} lily } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 15\%} nestled } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 10\%} sofia } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} leo } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} max } { {\fontsize{7}{7}\selectfont 8\%} owl } \\
Middle Eastern & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 27\%} ali } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 18\%} leila } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} layla } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} mysterious } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} dear } { {\fontsize{7}{7}\selectfont 5\%} tucked } \\
North American & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} lily } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} owl } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} fox } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} nestled } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} end } { {\fontsize{7}{7}\selectfont 5\%} thanked } \\
South American & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 19\%} maria } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 17\%} diego } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 15\%} monkey } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} waterfall } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} clearing } { {\fontsize{7}{7}\selectfont 5\%} branch } \\
\bottomrule\\


==> generated_unmasked/corr_story_text_lemmas_religion.tex <==
\null\\[-2.5em]
\multicolumn{2}{l}{\bf Religion} \\

Atheist & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} lily } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 8\%} realized } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} max } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} create } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} replied } { {\fontsize{7}{7}\selectfont 4\%} spent } \\
Buddhist & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} nestled } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 12\%} taught } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 11\%} mei } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} realized } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 8\%} replied } { {\fontsize{7}{7}\selectfont 8\%} let } \\
Christian & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} opened } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} lily } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} center } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} decided } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} branch } { {\fontsize{7}{7}\selectfont 4\%} followed } \\
Hindu & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} use } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} rohan } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} lived } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} returned } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} granted } { {\fontsize{7}{7}\selectfont 4\%} stumbled } \\
Jew & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 15\%} nestled } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} guide } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} began } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} dreaming } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} tucked } { {\fontsize{7}{7}\selectfont 4\%} said } \\
Muslim & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} aisha } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} amina } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} whispered } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} ali } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} dear } { {\fontsize{7}{7}\selectfont 4\%} clearing } \\
\bottomrule\\


==> generated_unmasked/corr_story_text_lemmas_role.tex <==
\null\\[-2.5em]
\multicolumn{2}{l}{\bf Role} \\

 & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 13\%} nestled } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 9\%} realized } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 8\%} taught } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} continued } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} replied } { {\fontsize{7}{7}\selectfont 5\%} explained } \\
father & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} use } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} rohan } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} lived } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} returned } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} granted } { {\fontsize{7}{7}\selectfont 4\%} stumbled } \\
mother & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} aisha } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 7\%} amina } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 6\%} whispered } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} ali } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} dear } { {\fontsize{7}{7}\selectfont 4\%} clearing } \\
parent & \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} opened } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} lily } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 5\%} center } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} decided } \makebox[22mm][l]{ {\fontsize{7}{7}\selectfont 4\%} branch } { {\fontsize{7}{7}\selectfont 4\%} followed } \\
\bottomrule\\


==> generated_unmasked/whole_story_word_prediction.tex <==
\begin{table*}[htbp]
\fontsize{8}{8}\selectfont
\begin{tabular}{p{2cm}l}
\toprule \\[-0.5em]
\input{generated_unmasked/corr_story_text_lemmas_gender.tex}
\input{generated_unmasked/corr_protagonist_gpt4_nationality_parent_group.tex}
\input{generated_unmasked/corr_story_text_lemmas_nationality_parent_developed.tex}
\input{generated_unmasked/corr_story_text_lemmas_ethnicity.tex}
\input{generated_unmasked/corr_story_text_lemmas_religion.tex}
\input{generated_unmasked/corr_story_text_lemmas_role.tex}
\end{tabular}
\vspace{-6mm}
\caption{Top words in the \textbf{text of the generated story} that correlate (Pearson) with the sociocultural factor.}
\label{tab:corr_bias_text}
\end{table*}


==> misc/old.tex <==

\begin{table*}[htbp]
\renewcommand{\arraystretch}{0.85}
\resizebox{\linewidth}{!}{
\fontsize{11.2pt}{11.2pt}\selectfont

\begin{tabular}{@{}l@{\hspace{2mm}}>{\small}l@{\hspace{1mm}}l}
\toprule
\multicolumn{3}{c}{Child gender} \\
\midrule
\input{generated/corr_bias_attr_gender.tex}
% to align
\vspace{18pt}
\end{tabular}
% 
\hfill
% 
\begin{tabular}{@{}l@{\hspace{2mm}}>{\small}l@{\hspace{1mm}}l}
\toprule
\multicolumn{3}{c}{Nationality} \\
\midrule
\input{generated/corr_bias_attr_nationality.tex} 
\end{tabular}
% 
\hfill
% 
\begin{tabular}{@{}l@{\hspace{2mm}}>{\small}l@{\hspace{1mm}}l}
\toprule
\multicolumn{3}{c}{Economy} \\
\midrule
\input{generated/corr_bias_attr_developing.tex} 
% to align
\vspace{4pt}
\end{tabular}
% 
\hfill
% 
\begin{tabular}{@{}l@{\hspace{2mm}}>{\small}l@{\hspace{1mm}}l}
\toprule
\multicolumn{3}{c}{Ethnicity} \\
\midrule
\input{generated/corr_bias_attr_race.tex} 
% to align
\vspace{4pt}
\end{tabular}
% 
\hfill
% 
\begin{tabular}{@{}l@{\hspace{2mm}}>{\small}l@{\hspace{1mm}}l}
\toprule
\multicolumn{3}{c}{Religion} \\
\midrule
\input{generated/corr_bias_attr_religion.tex} 
% to align
\vspace{4pt}
\end{tabular}
% 
\hfill
% 
\begin{tabular}{@{}l@{\hspace{2mm}}>{\small}l@{\hspace{1mm}}l}
\toprule
\multicolumn{3}{c}{Role} \\
\midrule
\input{generated/corr_bias_attr_role.tex} 
% to align
\vspace{20pt}
\end{tabular}
}

\vspace{-5mm}
\caption{Top words in \textbf{children attributes} in the generated story that correlate (Pearson) with the target variable, such as the child gender or parent's nationality. Obvious variables that correspond to the input, such as \textit{boy} are removed.}
\label{tab:corr_bias_attr}
\end{table*}



\begin{table*}[htbp]
\renewcommand{\arraystretch}{0.85}
\resizebox{\linewidth}{!}{
\fontsize{11.2pt}{11.2pt}\selectfont

\begin{tabular}{@{}l@{\hspace{2mm}}>{\small}l@{\hspace{1mm}}l}
\toprule
\multicolumn{3}{c}{Child gender} \\
\midrule
\input{generated/corr_bias_gender.tex}
% to align
\vspace{20pt}
\end{tabular}
% 
\hfill
% 
\begin{tabular}{@{}l@{\hspace{2mm}}>{\small}l@{\hspace{1mm}}l}
\toprule
\multicolumn{3}{c}{Nationality} \\
\midrule
\input{generated/corr_bias_nationality.tex} 
\end{tabular}
% 
\hfill
% 
\begin{tabular}{@{}l@{\hspace{2mm}}>{\small}l@{\hspace{1mm}}l}
\toprule
\multicolumn{3}{c}{Economy} \\
\midrule
\input{generated/corr_bias_developing.tex} 
% to align
\vspace{6pt}
\end{tabular}
% 
\hfill
% 
\begin{tabular}{@{}l@{\hspace{2mm}}>{\small}l@{\hspace{1mm}}l}
\toprule
\multicolumn{3}{c}{Ethnicity} \\
\midrule
\input{generated/corr_bias_race.tex} 
% to align
\vspace{6pt}
\end{tabular}
% 
\hfill
% 
\begin{tabular}{@{}l@{\hspace{2mm}}>{\small}l@{\hspace{1mm}}l}
\toprule
\multicolumn{3}{c}{Religion} \\
\midrule
\input{generated/corr_bias_religion.tex} 
% to align
\vspace{1pt}
\end{tabular}
% 
\hfill
% 
\begin{tabular}{@{}l@{\hspace{2mm}}>{\small}l@{\hspace{1mm}}l}
\toprule
\multicolumn{3}{c}{Role} \\
\midrule
\input{generated/corr_bias_role.tex} 
% to align
\vspace{20pt}
\end{tabular}
}



\vspace{-5mm}
\caption{Top words in the \textbf{text of the generated story} that correlate (Pearson) with the target variable, such as the child gender or parent's nationality. Words that refer to the childs attributes have been masked.}

\vilem{self-todo: try putting the attributes as rows}
\label{tab:corr_bias_text}
\end{table*}
